Neutrino Mixing and Leptogenesis in a $L_e-L_\mu-L_\tau$ model

We present a simple extension of the Standard Model with three right-handed neutrinos in a SUSY framework, with an additional U(1$)_\text{F}$ abelian flavor symmetry with a non standard leptonic charge $L_e-L_\mu-L_\tau$ for lepton doublets and arbitrary right-handed charges. We show that the model is able to reproduce the experimental values of the mixing angles of the PMNS matrix and of the $r=\Delta m_\text{sun}^2/\Delta m_\text{atm}^2$ ratio, with only a moderate fine tuning of the Lagrangian free parameters. The baryon asymmetry of the Universe is generated via thermal leptogenesis through CP-violating decays of the heavy right-handed neutrinos. We present a detailed numerical solution of the relevant Boltzmann equation accounting for the impact of the distribution of the asymmetry in the various lepton flavors.

==> Leptogenesis from flavor symmetry/unflavored.tex <==
\subsubsection*{Hierarchical scenario}
This alternative scenario is obtained by lowering the mass scale $\mathcal{M}$ down to a value of the order of $10^{13}\,\mbox{GeV}$, which brings to a hierarchical mass spectrum for the sterile neutrinos, with two heavy, almost degenerate, states with $M_1\simeq M_2\sim 10^{15}$ GeV, and a lighter one with $M_3\simeq 10^{13}$ GeV.
In this setup, the baryon asymmetry of the Universe can be generated through the conventional thermal leptogenesis only via the out-of-equilibrium decay of the lightest heavy neutrino. Similarly to the previous case, no flavor effects need to be accounted for. 
As discussed in \cite{Davidson:2008bu}, the latter becomes relevant when the rate of processes mediated by $\tau$, $\mu$ and $e$ exceeds the Hubble expansion rate. This occurs when the temperature of the Universe drops below, respectively:
\begin{equation}
\begin{aligned}
 T_\tau\simeq 5\cdot10^{11}\text{ GeV },\quad T_\mu\simeq 2\cdot10^{9}\text{ GeV },\quad T_e\simeq 4\cdot10^{4}\text{ GeV }\,.
\end{aligned}
\end{equation}
In the scenario under consideration we have $M_3\gg T_\tau \gg T_{\mu,e}$. Thus, we can work in the so-called \emph{unflavored regime}, in which the lightest neutrino decays via flavor blind processes. 
The baryon asymmetry can then be parametrized as: 
\begin{equation}
\eta_B\simeq 7.04\cdot 10^{-3}\,\varepsilon_3\, \eta_3\,,
\end{equation}
with $\eta_i$ as in eq.(\ref{efficiencyfactors}) and the unflavored CP-asymmetry as \cite{Blanchet:2012bk,Flanz:1994yx,Covi:1996wh,Buchmuller:1997yu}:
\begin{equation}
\varepsilon_{i}=\frac{1}{8\pi\left( Y^\dagger Y\right)_{ii}}\sum_{j\not=i} \text{Im}\left[\left( Y^\dagger Y\right)_{ij}^2\right]f\left[ \frac{M_j^2}{M_i^2}\right],
\end{equation}
where $x_j=M_j^2/M_i^2$ and the loop function is:
\begin{equation}
f[x]=\sqrt{x}\left[ 1-(1+x)\log\left( 1+\frac{1}{x}\right)+\frac{1}{1-x}\right]\,,
\end{equation}
that can be approximated to $f[x]\simeq -3/(2\sqrt{x})$ in the limit $x\gg 1$.
Expressing the elements of the Yukawa matrices in terms of the model parameters, we have:
\begin{equation}
\begin{aligned}
\varepsilon_{3}=\;f\left[ \frac{M_2^2}{M_3^2}\right]\frac{1}{8b^4\pi}\cdot \bigg \{ &\sin\left[ 2(\Sigma-\Omega)\right]\; \left(a^2b^2-2a^2(d_{23}^2+d_{33}^2)\right)+\\
&-2a\, b\, d_{22}\,d_{23}\sin\left[ \Theta-\Sigma+\Omega\right]+\\
&+2\,a\,b\,d_{32}\,d_{33}\sin\left[\Sigma-\Omega \right] +\mathcal{O}(\lambda^4)\bigg \}.
\end{aligned}
\end{equation}
Using the values in Tab.\ref{estimation_unflavored}, and noticing that $f\left[ M_2^2/M_3^2\right]\simeq 10^{-2}$, we obtain $\varepsilon_3\simeq 3.24\cdot 10^{-4}$.
\begin{table}[t]\centering
\centering
\begin{adjustbox}{width=0.42\textwidth, height= 1.25cm}
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
 $a$& $b$& $c$ & $d_{11}$ & $d_{22}$& $d_{23}$&$d_{31}$&$d_{32}$\\
\hline
1.18&1.07 & 1.65&1.99&1.95&1.88&1.82&1.71\\
\hline
\hline
 $d_{33}$& $m$ & $\Sigma$ & $\Omega$& $\Theta$&$\Phi$&$Z$&$W$\\
\hline
1.83& 1.50 & 0.39& 1.02 & 4.10&5.11&1.41&159.97\\
\hline
\end{tabular}
\end{adjustbox}
\caption{\it Set of parameter assignments which lead to a final baryon asymmetry close to the cosmological observations. See text for further details.}
\label{estimation_unflavored}
\end{table}
The corresponding efficiency factor $\eta_{3}$ can be simply approximated to:
\begin{equation}
    \eta_3\simeq 3.6\cdot 10^{-4}\left(\frac{Z}{b^2} + O(\lambda^4)\right)\simeq 4.3\cdot 10^{-4}\,,
\end{equation}
for the assignations in Tab.\ref{estimation_unflavored}. The efficiency factor can be converted to the baryon asymmetry parameter $\eta_B$:
\begin{equation}
    \eta_B\simeq 7.04\times10^{-3}\left[ \varepsilon_{3}\eta_{3}\right]\approx 9.5 \times 10^{-10}\,,
\end{equation}
very close to the experimentally favoured value.
Also in this case, we have verified the goodness of our analytical approximations by solving a suitable set of Boltzmann equations, which take the form:
\begin{equation}
\begin{aligned}
\frac{dN_3}{dz}=&-\left(D_3-S_3\right)\left( N_3-N_3^\text{eq}\right)\,,\\
\frac{dN_{B-L}}{dz}=&\;\varepsilon_{3}D_3\left( N_3-N_3^\text{eq}\right)-W_3N_{B-L}\,.
\end{aligned}
\end{equation}
From the parameter choices in Tab.\ref{estimation_unflavored}, we get the following Yukawa matrix :
\begin{equation}
\hat{\text{Y}}=\begin{pmatrix}0.39-1.07i&-0.71-0.32i&-0.44-0.70i\\
											-0.52+1.07i&-0.84-0.32i&-0.36-0.59i\\
											+0.08825-0.00004i&+0.0821-0.0003i &+0.0881-0.0007i\end{pmatrix}\,.
\end{equation}
Notice that the imaginary parts of the third row is suppressed by a factor proportional to $Z/W$. \\
This choice corresponds to the CP-violation parameter $\varepsilon_{3}=4.3\cdot 10^{-4}$.
\begin{figure}[tb]
\centering
\includegraphics[width=11cm, height=6cm]{hierarchyNew.pdf}
\caption{\it Evolution of the $B-L$ symmetry in the {\it hierarchical scenario.} The color code is the same as in fig.\ref{fig:B-LResonance}.}
\label{fig:unFlavored}
\end{figure}
For the benchmark values under consideration, the numerical solution of the Boltzmann's equations is shown in fig.\ref{fig:unFlavored} and gives:
\begin{equation}
\begin{aligned}
N_{B-L}(\infty)=&\;2.75\cdot10^{-8}\,,\\
\eta_B=&\;3.96\cdot10^{-10}\,,
\end{aligned}
\end{equation}
confirming what we expected from the simplified analytical analysis.
It is interesting to notice that, contrary to the resonant regime, in the hierarchical scenario it is possible to find a parameter assignation leading to viable leptogenesis without imposing a fine tuning on the CP violating phases.
